Long-Time Dynamics of KdV Solitary Waves over a Variable Bottom

We study the variable bottom generalized Korteweg-de Vries (bKdV) equation dt u=-dx(dx^2 u+f(u)-b(t,x)u), where f is a nonlinearity and b is a small, bounded and slowly varying function related to the varying depth of a channel of water. Many variable coefficient KdV-type equations, including the variable coefficient, variable bottom KdV equation, can be rescaled into the bKdV. We study the long time behaviour of solutions with initial conditions close to a stable, b=0 solitary wave. We prove that for long time intervals, such solutions have the form of the solitary wave, whose centre and scale evolve according to a certain dynamical law involving the function b(t,x), plus an H^1-small fluctuation.

==> Formatting.tex <==
\makeatletter
% catches author and title for the headers, must be before \maketitle
% that clears the
% variables \@author and \@title

\def\catchNameTitle{
\global\let\Author\@author
\global\let\Title\@title
}

% creates a string with the time now.
\def\timenow{%
  \@tempcnta=\time \divide\@tempcnta by 60 \number\@tempcnta:\multiply
  \@tempcnta by 60 \@tempcntb=\time \advance\@tempcntb by -\@tempcnta
  \ifnum\@tempcntb <10 0\number\@tempcntb\else\number\@tempcntb\fi}

% creates a string with todays date Swedish version
\def\TODAY{\number\year-\ifcase\month\or 01\or 02\or 03\or 04\or 05\or
    06\or 07\or 08\or 09\or 10\or 11\or 12\fi-\ifnum\day<10 0\number\day\else \number\day\fi}

% substitute for markboth or simular commands sets the page with #1
%to #4 one in each corner on every page

\newcommand{\MarkAll}[4]{
\renewcommand{\ps@myheadings}{
\renewcommand{\@oddhead}{{\scriptsize #1 \hfil #2}}
\renewcommand{\@evenhead}{\@oddhead}
\renewcommand{\@evenfoot}{{\scriptsize #3}\hfil
    \textrm{\thepage}\hfil{\scriptsize #4}}
\renewcommand{\@oddfoot}{\@evenfoot}}
}

\def\NOW{\TODAY;\timenow}

\newcommand{\DRAFT}{
\renewcommand{\@evenhead}{\hfil DRAFT \hfil}
\renewcommand{\@oddhead}{\@evenhead}
}

\newcommand{\NowFootNum}{
\renewcommand{\@evenfoot}{{\scriptsize \jobname.tex}\hfil
    \textrm{\thepage}\hfil {\scriptsize \NOW}}
\renewcommand{\@oddfoot}{\@evenfoot}
}

\newcommand{\NowFoot}{
\renewcommand{\@evenfoot}{{\scriptsize \jobname.tex} {\scriptsize \NOW}}
\renewcommand{\@oddfoot}{\@evenfoot}
}


\def\fixNumberingInArticle{
\@addtoreset{figure}{section}
%\@addtoreset{equation}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
%\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\theequation}{\arabic{equation}}
%\renewcommand{\theenumi}{\arabic{enumi}}
}

\def\fixNumberingInAppendix{
\setcounter{section}{0}
\renewcommand{\theequation}{\Alph{section}.\arabic{equation}}
\renewcommand{\thesection}{\Alph{section}}
\setcounter{equation}{0}
}



\makeatother

